Almost Linear Convergence under Minimal Score Assumptions: Quantized Transition Diffusion

Continuous diffusion models have demonstrated remarkable performance in data generation across various domains, yet their efficiency remains constrained by two critical limitations: (1) the local adjacency structure of the forward Markov process, which restricts long-range transitions in the data space, and (2) inherent biases introduced during the simulation of time-inhomogeneous reverse denoising processes. To address these challenges, we propose Quantized Transition Diffusion (QTD), a novel approach that integrates data quantization with discrete diffusion dynamics. Our method first transforms the continuous data distribution $p_*$ into a discrete one $q_*$ via histogram approximation and binary encoding, enabling efficient representation in a structured discrete latent space. We then design a continuous-time Markov chain (CTMC) with Hamming distance-based transitions as the forward process, which inherently supports long-range movements in the original data space. For reverse-time sampling, we introduce a \textit{truncated uniformization} technique to simulate the reverse CTMC, which can provably provide unbiased generation from $q_*$ under minimal score assumptions. Through a novel KL dynamic analysis of the reverse CTMC, we prove that QTD can generate samples with $O(d\ln^2(d/\epsilon))$ score evaluations in expectation to approximate the $d$--dimensional target distribution $p_*$ within an $\epsilon$ error tolerance. Our method not only establishes state-of-the-art inference efficiency but also advances the theoretical foundations of diffusion-based generative modeling by unifying discrete and continuous diffusion paradigms.

==> 0_config/init_load.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input

%-----------------------------------
\pdfoutput=1

\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm,amsfonts}
\usepackage{array}
\usepackage{authblk}
\usepackage{babel}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{colortbl}% http://ctan.org/pkg/xcolor
\usepackage{enumitem}
\usepackage[T1]{fontenc}    
\usepackage{framed}
\usepackage{graphicx}
\usepackage[linkcolor=red]{hyperref}
\usepackage{indentfirst}
\usepackage[utf8]{inputenc}
\usepackage{lipsum}        
\usepackage{makecell}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{xparse}
% \usepackage{subcaption}
\usepackage[framemethod=default]{mdframed}
\usepackage{microtype}     
\usepackage{multicol}
\usepackage{multirow}
%\usepackage{natbib}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{tablefootnote}
\usepackage{url}            % simple URL typesetting
\usepackage{wrapfig,lipsum}
\usepackage{xcolor}         % colors
\usepackage{xspace}

\usepackage{subfigure}
\usepackage[capitalize,noabbrev]{cleveref}


\usepackage{doi}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
% \renewcommand{\baselinestretch}{1.1}



==> 0_figures/discrete_jump.tex <==
\begin{tikzpicture}





\filldraw (0,-2.5) circle (0.05); \node at (-0.2, -2.8) {$0$}; 
\draw[-]  (0,-2.5)--(2,-2.5);
\filldraw (2,-2.5) circle (0.05); \node at (1.8, -2.8) {$1$}; 
\draw[-] (2,-2.5)--(4,-2.5);
\filldraw (4,-2.5) circle (0.05); \node at (3.8, -2.8) {$2$}; 
\draw[-] (4,-2.5)--(6,-2.5);
\filldraw (6,-2.5) circle (0.05);\node at (5.8, -2.8) {$3$};
\draw[-] (6,-2.5)--(8,-2.5);
\filldraw (8,-2.5) circle (0.05); \node at (7.8, -2.8) {$4$}; 
\draw[-]  (8,-2.5)--(10,-2.5);
\filldraw (10,-2.5) circle (0.05); \node at (9.8, -2.8) {$5$}; 
\draw[-] (10,-2.5)--(12, -2.5);
\filldraw (12,-2.5) circle (0.05); \node at (11.8, -2.8) {$6$}; 
\draw[-] (12,-2.5)--(14, -2.5);
\filldraw (14,-2.5) circle (0.05); \node at (13.8, -2.8) {$7$}; 

\draw[-latex, blue] (0,-2.5)..controls (1, -1.9)..(2,-2.5);

\draw[-latex, blue] (0,-2.5)..controls (2, -0.9)..(4,-2.5);

\draw[-latex, blue] (0,-2.5)..controls (4, 0.5)..(8,-2.5);

\draw[-latex, red] (10,-2.5)..controls (9, -3.1)..(8,-2.5);

\draw[-latex, red] (10,-2.5)..controls (6, -4.5)..(2,-2.5);

\draw[-latex, red] (10,-2.5)..controls (12, -0.9)..(14,-2.5);


\end{tikzpicture}
